Noise-Free Explanation for Driving Action Prediction

Although attention mechanisms have achieved considerable progress in Transformer-based architectures across various Artificial Intelligence (AI) domains, their inner workings remain to be explored. Existing explainable methods have different emphases but are rather one-sided. They primarily analyse the attention mechanisms or gradient-based attribution while neglecting the magnitudes of input feature values or the skip-connection module. Moreover, they inevitably bring spurious noisy pixel attributions unrelated to the model's decision, hindering humans' trust in the spotted visualization result. Hence, we propose an easy-to-implement but effective way to remedy this flaw: Smooth Noise Norm Attention (SNNA). We weigh the attention by the norm of the transformed value vector and guide the label-specific signal with the attention gradient, then randomly sample the input perturbations and average the corresponding gradients to produce noise-free attribution. Instead of evaluating the explanation method on the binary or multi-class classification tasks like in previous works, we explore the more complex multi-label classification scenario in this work, i.e., the driving action prediction task, and trained a model for it specifically. Both qualitative and quantitative evaluation results show the superiority of SNNA compared to other SOTA attention-based explainable methods in generating a clearer visual explanation map and ranking the input pixel importance.

==> note.tex <==
% \begin{itemize}
%     \item \href{https://doc.bdd100k.com/download.html}{BDD100K}
%     \item \href{https://www.a2d2.audi/a2d2/en/tutorial.html}{A2D2}
%     \item \href{https://usa.honda-ri.com/dataset-download?requestKey=01054424-8D4338ZG}{HDD}
%     \item \href{https://europe.naverlabs.com/research/computer-vision/proxy-virtual-worlds-vkitti-1/}{KITTI}
%     \item \href{https://waymo.com/open/download/}{Waymo}
% \end{itemize}

% In the past year, seminal works have successfully adopted Transformers for computer vision problems,  such as image classification and detection. Using a large amount of unsupervised data offers a great opportunity to pretraining these rich Transformer-based image representations.
% Beyond driving performance, interpretability is a major concern for autonomous driving. 
% overlooks the interactions among features.

% These noises may indeed reflect the true behaviour of the gradients of the deep neural model: as the networks get deeper, the gradients across the input space fluctuate more sharply, resembling white noise, which is described as the shattering gradient problem.

% Momentum teacher\cite{he2020momentum} and multi-crop training \cite{caron2020unsupervised} are critical components for the success of DINO.

% By setting the token value of a specific patch to zero, it removes the information associated with that patch from the input representation. 

Our method uses norm-weighted attention $A^{l}\|\hat{\boldsymbol{v}^l} \Vert$ of each attention layer to update the relevancy maps. 

Since each attention layer comprises h heads, Note that as each attention head differs in importance and relevance\cite{voita2019analyzing}, as is shown in Figure \ref{fig:multi-head}. thus, it is not wise to directly average across heads of $A^{l}\|\hat{\boldsymbol{v}^l} \Vert$. So, we use attention gradients to average across heads. The final averaged attention map $\Bar{A}^l$ of our method is then defined as follows:

% However, In ViT, the representation of a token is highly dependent on its interactions with all other tokens. We may underestimate their importance by zeroing out attention weights for specific tokens due to the complex, multi-layer interactions that can compensate for their absence in later layers.

% \cite{hofmarcher2019visual} propose a semantic segmentation model that employs pixel-wise classification to elucidate the underlying real-time perception of the environment. 

% Kim and Canny\cite{kim2017interpretable} utilize a causal attention model integrated with saliency filtering to identify input regions influencing the output, particularly in steering control. Building upon this work, Kim et al.\cite{kim2018textual} introduce textual explanations through an attention-based video-to-text mechanism, producing "explanations" for the decisive actions of self-driving vehicles. Xu et al.\cite{xu2020explainable} propose object-induced actions with explanations for autonomous car predictions, Kim et al.\cite{kim2020advisable} propose an approach that integrates human advice to facilitate vehicle control learning, enabling the system to generate explanations for decisive actions based on sensed operational surroundings. Li et al.\cite{li2020make} present a method to identify risk objects influencing specific driving behaviours. 

% Their approach demonstrates that randomly eliminating certain objects from the scene alters driving decisions, such as transitioning from a "Stop" to a "Go" command. 

% where $\boldsymbol{Z}^{0}$ is the input patches embedding, $\boldsymbol{z^{0}_i} = \boldsymbol{E(x^{0}_i)}$, $i \in \{1,...,n\}$, $\boldsymbol{E}$ is the function of Patch Embedding and Position Embedding. 

% \begin{center}
% \begin{table}[h]
%      \resizebox{0.9 \columnwidth}{!}
%      {
%         \begin{tabular}{cc}
%         \hline
%         \textbf{Method} & \textbf{Expression} \\
%         \hline
%         Raw Attention & $A^{L}$ \\
%         % Raw Gradient & $\nabla A^{L}$ \\
%         % Attention Rollout & $A^{1}\cdot A^{2} \cdots A^{L}$ \\
%         Attention $\odot$ Gradient & $ A^L \odot \nabla {A^L}$ \\
%         Attention InputNorm & $\|A^L\hat{v}^L\Vert$  \\
%         Generic Attention &  $\Bar{A}=\mathbb{E_h}((A \odot \nabla A)^{+})$ \\
%         Attention IG &  $\Bar{A} \odot IG $ \\
%         \hline
%         \end{tabular}
%     }
%     \caption{Baseline Methods Compared in this paper, $A$ denotes the raw attention weights, $A^L$ on behalf of the last layer attention, $\Bar{A}$ means head average attention, IG is Integrated Gradient. }
%     \label{table:baseline }
%     % \vspace{1em}
% \end{table}
% \end{center}

% \footnote{$h$ consists of a 3-layer multi-layer perceptron (MLP) with hidden dimension 2048 followed by $l_2$ normalizations and a weight normalized fully connected layer with the output dimensions K}

% In the real world, most of the time, driving involves simply “moving forward”, and only a few times when we need to make changes in a relatively short period. 


% \paragraph{BackPropogration-based}
% Supported by the theory of Deep Taylor Decomposition (DTD) \cite{montavon2017explaining}, Layer-wise relevance propagation (LRP)\cite{binder2016layer}  based methods recursively decompose the decision made by the network into the initial layer's contributions to the elements of the network’s input. PartialLRP \cite{voita2019analyzing} uses LRP to compute the relative importance scores for each attention head in the last Transformer layer and then averages them across heads as explanations. However, this approach is limited by only providing partial information on each self-attention head’s relevance; no relevance score is propagated back to the input. TransAtt \cite{chefer2021transformer} combines the gradients with LRP and attention maps along a rolling-out path and eliminates the negative components in each attention block. Though gradients in a way reflect the direct influence to the final objective, involving them intuitively and masking the negatives in each attention block risk losing useful information from relevance scores or attention maps.

% \begin{center}
% \begin{table}[h]
%      \resizebox{0.9 \columnwidth}{!}
%      {
%         \begin{tabular}{cc}
%         \hline
%         \textbf{Method} & \textbf{Expression} \\
%         \hline
%         RawAtt & $A^{L}$ \\
%         AttGrad & $ A^L \odot \nabla {A^L}$ \\
%         AttIN & $\|A^L\hat{v}^L\Vert$  \\
%         GenericAtt & $A^{*} = \prod_{i=1}^L(\mathbb{E_h}(A^i \odot \nabla A^i)^{+} + \mathbb{1})$ \\
%         AttIG &  $ A^{*} \odot IG $ \\
%         \hline
%         \end{tabular}
%     }
%     \caption{Baseline Attention based Methods Compared in this paper, $A$ denotes the raw attention weights, $A^L$ on behalf of the last layer attention, IG is Integrated Gradient. }
%     \label{table:baseline}
%     % \vspace{-1em}
% \end{table}
% \end{center}

% The features used in downstream tasks are the backbone $f$ output.
% We refer interested readers to \cite{caron2021emerging} for more details regarding DINO.

% The self-attention mechanism establishes connections between each token and the [CLS] token, with the strength of these connections indicating each token's contribution to classification. However, attention values represent only one facet of the Transformer network or the self-attention head.

% The performance of XAI methods relies on the input and model prediction results. Whether the classification accuracy of a classifier will affect the performance of XAI methods remains to be investigated.
